Two-Stream AMTnet for Action Detection

In this paper, we propose Two-Stream AMTnet, which leverages recent advances in video-based action representation[1] and incremental action tube generation[2]. Majority of the present action detectors follow a frame-based representation, a late-fusion followed by an offline action tube building steps. These are sub-optimal as: frame-based features barely encode the temporal relations; late-fusion restricts the network to learn robust spatiotemporal features; and finally, an offline action tube generation is not suitable for many real-world problems such as autonomous driving, human-robot interaction to name a few. The key contributions of this work are: (1) combining AMTnet's 3D proposal architecture with an online action tube generation technique which allows the model to learn stronger temporal features needed for accurate action detection and facilitates running inference online; (2) an efficient fusion technique allowing the deep network to learn strong spatiotemporal action representations. This is achieved by augmenting the previous Action Micro-Tube (AMTnet) action detection framework in three distinct ways: by adding a parallel motion stIn this paper, we propose a new deep neural network architecture for online action detection, termed ream to the original appearance one in AMTnet; (2) in opposition to state-of-the-art action detectors which train appearance and motion streams separately, and use a test time late fusion scheme to fuse RGB and flow cues, by jointly training both streams in an end-to-end fashion and merging RGB and optical flow features at training time; (3) by introducing an online action tube generation algorithm which works at video-level, and in real-time (when exploiting only appearance features). Two-Stream AMTnet exhibits superior action detection performance over state-of-the-art approaches on the standard action detection benchmarks.

==> text/1_intro.old.tex <==
% conributions
% adding motion in amtnet improve perfornamce
% soa dont support end to end training
% can not learn pixel-wise correspondences between app. and motion features
% online incremental tube generaion

% \section{Introduction} \label{sec:intro}
\IEEEraisesectionheading{\section{Introduction}\label{sec:intro}}
% -----------------------  action detection based on frame level object detectors  ---------------------------------------------------------------------
\IEEEPARstart{S}{patiotemporal} human action detection in videos is one of the core challenging problems in computer vision.
In recent years, notable progress has been observed in this area~\cite{Georgia-2015a,Weinzaepfel-2015,peng2016eccv,Saha2016,kalogeiton2017action,hou2017tube}.
However, some common limitations with these approaches are as follows.
%---------------------------------------------------------------------
\textbf{(a)} Firslty, they follow a \emph{frame based} feature representation (except~\cite{kalogeiton2017action,hou2017tube}) suitable for image level detection task such as object detection in images~\cite{girshick2016region,girshick2015fast}, but limiting these models to learn only spatial or appearance based features and not the sptiotemporal encoding required for action detection in videos, i.e., these architectures are not able to take full advantage of temporal information~\cite{saha2017amtnet} present in videos.
%---------------------------------------------------------------------
\textbf{(b)} Secondly, they train appearance and motion streams separately and fuse the appearance and motion cues at \emph{test time}, restricting these models to learn the complementary aspects of appearance and motion cues during training time, i.e. registration of spatial cue with temporal cue and how these cues evolve over time~\cite{Feichtenhofer_2016_CVPR}. 
As two separate networks (appearance and motion streams) are trained independently, the optimisation step is \emph{disjoint}, and thus, these frameworks can not be trained in an \emph{end-to-end} fashion.
%---------------------------------------------------------------------
\textbf{(c)} As a third limitation, these action detectors~\cite{Georgia-2015a,Weinzaepfel-2015,peng2016eccv,Saha2016} are suitable for \emph{offline} processing, i.e., they assume that the entire video (taken as a 3D block of pixels) is available ahead of time in order to detect action instances.
Although, \cite{kalogeiton2017action,hou2017tube} use an online tube generation algorithm, it is limited by stacking $k$ video frames which is expensive and not suitable for real-time applications.
For such a detector to be applicable to real-world scenarios such as video surveillance and human-robot interaction, video frames need to be processed online, i.e., 
generating action tubes incrementally over time as a burst of frames arrive.
Besides, the testtime \emph{detection speeds} of these detectors are slow and not suitable for real-world deployment.
%---------------------------------------------------------------------
\textbf{(d)} Finally, action detection methods such as~\cite{kalogeiton2017action,hou2017tube} require dense ground truth annotation for network training: bounding-box annotation is required for $k$ consecutive video frames, where $k$ is the number of frames in a training example. 
Kalogeiton~\etal~\cite{kalogeiton2017action} use $k=6$ whereas for Hou~\etal~\cite{hou2017tube} $k=8$.
Generating such dense bounding box annotation for long video sequences is highly expensive and impractical ~\cite{daly2016weinzaepfel,ava2017gu}.
The latest generation action detection benchmarks DALY~\cite{daly2016weinzaepfel} and AVA~\cite{ava2017gu}, in contrast, provide sparse bounding-box annotations.
More specifically,  DALY has $1$ to $5$ frames bounding box annotation per action instance irrespective of the duration of an instance, whereas AVA has only one frame annotation per second.
% \emph{This motivates the design of a deep network able to handle sparse annotations, while still being able to predict micro-tubes over multiple frames}.


In this work, we aim to address these aforementioned limitations in the existing action detectors.
We propose an action detection framework (Section~\ref{sec:amtnet-flow-offline}~\&~\ref{sec:amtnet-flow-online}) which follows a \emph{video based} feature representation (in place of a \emph{frame based} one) which can encode spatiotemporal patterns of human actions in videos. 
For this, we adapt the recent AMTnet~\cite{saha2017amtnet} deep network architecture. The main reasons for selecting AMTnet over \cite{kalogeiton2017action,hou2017tube} are:
(a) AMTnet requires only a pair of successive video frames for action representation as opposed to \cite{kalogeiton2017action,hou2017tube} which requires $k$ consecutive video frames ($k=6$ for \cite{kalogeiton2017action} and $k=8$ for \cite{hou2017tube}) which is computationally expensive and not suitable for real-time applications. 
(b) Unlike~\cite{kalogeiton2017action,hou2017tube}, AMTnet requires \emph{pairs} of successive frames $(f_t, f_{t+\Delta})$, eliminating the need for dense training annotation when $\Delta$ is large or arbitrary DALY~\cite{daly2016weinzaepfel}.
In Section~\ref{sec:exp:impace-of-diff-delta}, we show that the proposed action detection framework behaves gracefully when trained on larger deltas (e.g. $\Delta=\{ 8, 16\}$) achieving similar video-mAPs as models trained on smaller deltas (e.g. $\Delta=\{2, 4\}$).


Furthermore, we extend the AMTnet architecture by adding a motion stream allowing:
(1) an end-to-end training of both the streams (appearance and motion), and
(2) a train time feature (RGB and flow) fusion.
In Section~\ref{sec:exp:impace-of-feat-fusion}, we show that our train-time RGB and optical flow based convolutional feature fusion improves the video-mAP over the widely used test-time late fusion
~\cite{Georgia-2015a,Weinzaepfel-2015,peng2016eccv,Saha2016,kalogeiton2017action,hou2017tube}.


%--------------------
Finally, unlike previous offline tube generation approaches~\cite{Georgia-2015a,Saha2016,peng2016eccv,Weinzaepfel-2015}, 
we propose an online algorithm which incrementally build action tubes by linking micro-tubes in time.
In Section~\ref{sec:exp:impace-of-online-algo}, we show that our online algorithm outperforms the existing offline tube generation approaches.



%-------- overview ---------
\textbf{Overview of the approach}. 
% Our proposed network architectures (Fig.~\ref{fig:amtnet-flow-online}) employ and adapt the architectural components of AMTnet~\cite{saha2017amtnet}.
% Firstly, we add a motion stream to the existing AMTnet architecture and introduce a train time RGB and optical flow feature fusion scheme (Section~\ref{sec:amtnet-flow-offline-featfusion}~\&~\ref{sec:amtnet-flow-online-featfusion}).
% We quantitatively demonstrate that the new deep network architecture outperforms the baseline AMTnet (Section~\ref{sec:exp:subsec:offline:motstream}).
% We termed the new network as \emph{``AMTnet-Flow offline''}.

To generate the final action tubes we adapt the offline micro-tube linking algorithm of~\cite{saha2017amtnet} (Section~\ref{sec:amtnet-flow-offline-tubegen}).
%----------
AMTnet follows a Faster-RCNN network architecture which takes relatively large computing time and resources, and thus, not suitable for designing an online real-time action detection pipeline. 
We replace the Faster-RCNN network architecture~\cite{ren2015faster} with faster SSD~\cite{liu2016ssd} network and design an online version of AMTnet-Flow (Section~\ref{sec:amtnet-flow-online}).
We termed this new network as \emph{``AMTnet-Flow online''}. 
SSD eliminates the need of a separate RPN network (as in Faster-RCNN) for generating region proposals, and thus, takes less computing time both at train and test time. 
Unlike Faster-RCNN in which representation is learnt from conv feature maps at single scale, an SSD network learns representation from conv feature maps at multiple scales, thus, it is robust to scale changes (i.e. able to detect very smaller objects/actions in videos/images). Another exciting property of SSD is: it learns invariant representation using a rich set of data augmentation schemes in place of a standard ROI (region of interest) max-pooling operation as in Faster-RCNN. 
Following the online action detection approach~\cite{singh2016online}, we design our AMTnet-Flow online using SSD.
To incrementally link the detection micro-tubes in an online fasion, we adapts the online tube generation algorithm of~\cite{singh2016online}.
Unlike~\cite{singh2016online} in which frame level detections are incrementally link in time, our online algorithm incrementally links detection micro-tubes at test time (Section~\ref{sec:online:subsec:tubegen}).


\begin{figure}[!ht]
{
\centering
\includegraphics[width=0.45\textwidth]{figures/intro/3d_prop_micro_tube.pdf}
\caption
{
\textbf{(a)}: AMTnet's video based action representation in which a regression layer learns a transformation to map a 3D region proposal (in red) to a ground truth micro-tube (in green);
\textbf{(b)}: Temporally linking detection micro-tubes at test time.
}
\label{sec:intro:fig:3dp_mt}
}
\end{figure} 


Before we proceed further, we would like to explain the concepts of \emph{3D region proposals} and  \emph{action micro-tubes} with an example which helps the readers to understand the action detection framework presented in this paper.
Consider Figure~\ref{sec:intro:fig:3dp_mt} (a) where a \emph{``diving''} action spans two successive (but necessarily consecutive) video frames $f_{t}$ and $f_{t+\Delta}$.
In this case, a ground truth action \textbf{micro-tube} ( i.e. a pair of ground truth bounding boxes belongs to frames $f_{t}$ and $f_{t+\Delta}$ respectively) is shown in green.
One of the best matched \textbf{3D region proposals} (i.e. a pair of anchor/default boxes which has high mean overlap with the corresponding ground truth boxes) is shown in red.
At the time of training AMTnet network, the regression layer learns a transformation to map the 3D region proposal (red) to the ground truth micro-tube (green).   

Unlike frame based action detection methods~\cite{Georgia-2015a,Weinzaepfel-2015,Saha2016,peng2016eccv} which output detection bounding-boxes at test-time, an action detection model trained on video based feature representation outputs detection micro-tubes.
Temporally linking detection micro-tubes is faster than linking frame level detections (for more details, please refer to Section~\ref{}).    
Figure~\ref{sec:intro:fig:3dp_mt} (b) shows the temporal linking of the action micro-tubes extracted during test time.    \\


\textbf{Contributions.} 
The main contributions of this paper are as follows.
\textbf{(1)}  A video based representation allows spatiotemporal feature encoding required for action detection in videos and also supports sparse bounding box annotations (Section~\ref{sec:amtnet-flow-offline}~\&~\ref{sec:amtnet-flow-online}).
\textbf{(2)} A training time RGB and optical flow fusion scheme allowing the network to learn the complementary aspects of appearance and motion cues, and also facilitates a joint training optimisation of both the appearance and motion streams in an end-to-end fashion (Section~\ref{sec:amtnet-flow-offline-featfusion}~\&~\ref{sec:amtnet-flow-online-featfusion}).
In contrast, the previous approaches~\cite{Georgia-2015a,Weinzaepfel-2015,peng2016eccv,Saha2016,kalogeiton2017action,hou2017tube} follow a disjoint training optimisation, i.e., the appearance and motion streams are trained separately and the fusion is done at test time (a late fusion strategy).
We quantitatively show that our train time conv feature fusion performs better than the test time late fusion scheme (Section~\ref{sec:exp:online}). % TODO -- refer the section in exp section where Guru has show better online results on JHMDB
\textbf{(3)} an online action detection pipeline which outperforms the state-of-the-art offline approaches~\cite{Georgia-2015a,Weinzaepfel-2015,peng2016eccv,Saha2016,kalogeiton2017action,hou2017tube}  (Section~\ref{sec:exp:online}).

Beside these aforementioned core contributions, we quantitatively demonstrate that the action detection performance can be significantly improved by adding a parallel motion stream to the existing AMTnet model (Section~\ref{sec:exp:subsec:offline:motstream}).
We also train AMTnet-Flow (offline and online models) on both nearby and widely separated frame pairs (i.e. pairs having short and long inter-frame distance), and at the test time, we improve the detection speed significantly by extracting action micro-tubes on long distance pairs (Section~\ref{sec:exp:subsec:offline:subsub:tubegen}).
% \label{sec:exp:subsec:offline:subsub:tubegen}
% \label{sec:exp:subsec:offline:subsub:boxinterpol}
At test time to extract longer detection micro-tubes, we propose an efficient \emph{``box interpolation algorithm''} (Section~\ref{sec:exp:subsec:offline:subsub:boxinterpol}) which populates the missing bounding boxes for intermediate frames by using linear interpolation of box coordinates.






% (1) a novel deep netowrk architecture which facilitates video based feature representation satiable for action detection in videos and supports datasets with sparse bounding box annotations;
% (2) a train time RGB and optical flow feature fusion scheme allowing the network to learn the complementary aspects of appearance and motion cues during training time;
% (3) an online real-time action detection pipeline.


\iffalse
Following from the AMTnet work~\cite{saha2017amtnet}, here we extend the AMTnet deep architecture to improve both action detection performance and speed.
The main contributions of this paper is as follows. 
\textbf{(a)} We significantly improve the action detection performance of AMTnet by incorporating optical flow features (\S~\ref{}). 
We name this new deep network as \emph{``AMTnet-Flow''} (\S~\ref{}). 
\textbf{(b)} Unlike AMTnet, we train AMTnet-Flow on both nearby and widely separated frame pairs (i.e. pairs having short and long inter-frame distance), and at the test time, we improve the detection speed significantly by extracting action micro-tubes on long distance pairs (Section~\ref{ch:bmvc2017:sec:train_data_sampl_scheme}).
At test time to extract longer detection micro-tubes, we propose an efficient \emph{``box interpolation algorithm''} (Section~\ref{ch:bmvc2017:sec:bbiatg:subsec:box_interpolation}) which populates the missing bounding boxes for intermediate frames by using linear interpolation of box coordinates.
For temporal linking of longer micro-tubes (Section~\ref{ch:bmvc2017:sec:bbiatg:subsec:tube_gen}), we modify the micro-tube linking algorithm (Section~\ref{ch:iccv2017:sec:action-tube}) which further 
speeds up the tube generation step (Section~\ref{ch:bmvc2017:sec:eval:subsec:impact_tube_gen_algo}).
\textbf{(c)} Unlike the test time fusion approach \cite{Georgia-2015a,Weinzaepfel-2015,Saha2016,peng2016eccv}, our new train time CNN feature fusion scheme allows the network to learn the pixel-wise
correspondences between appearance and motion features~\cite{Feichtenhofer_2016_CVPR}.
\fi

%-------- overview ---------
% \textbf{Overview of the approach}. 
% offline -  amtnet + flow + train time fusion + offline tube generation -- this is baseline
% online - amtnet using ssd following guru iccv paper + guru online algo + train time fusion

\iffalse
To address the first limitation and to learn a video based feature encoding, optical flow features~\cite{Georgia-2015a} are heavily exploited~\cite{Georgia-2015a,Weinzaepfel-2015,peng2016eccv,Saha2016}.
Among these, Peng \etal's~\cite{peng2016eccv} approach shows superior detection performance.
However, we argue that their approach is computationally expensive 
in terms of both computing time and cost (\S~\ref{}).% TODO refer the discussion section

In contrast, we train both the appearance and motion streams jointly and the proposed approach follows a \emph{single-stage} training i.e. our network requires only one time training and does not require any finetuning as in~\cite{peng2016eccv}.
At test time, the network receives a pair of successive video frames ($f_t$ and $f_{t+\Delta}$ where $\Delta=4$, see Fig.~\ref{fig:box-intrpl_mt_linking} (a)) as input, and predicts pairs of bounding boxes (called action micro-tubes~\cite{saha2017amtnet}, see Fig.~\ref{fig:box-intrpl_mt_linking} (b)) which are linked in time. 
Thus, our model requires to process only $50\%$ of the entire video frames which significantly reduces the computing time and cost.
Moreover, we follow single-scale training and testing schemes i.e., we use each video frame only once as compared to~\cite{peng2016eccv} which uses one frame thrice (at 3 different scales).
With these aforementioned properties i.e., an end-to-end trainable network and relatively low computing requirements, the proposed approach outperforms~\cite{peng2016eccv} at higher IoU thresholds ($\delta$) (Table~\ref{table:com-soa-ucf101}) on one of the largest action detection datasets (UCF-101-24~\cite{soomro-2012}) to date.\\
\fi




\iffalse
\begin{figure*}[!t]
{
\centering
\includegraphics[width=0.99\textwidth]{figures/intro/pipelineOverview.pdf}
\caption{Overview of the proposed action detection framework.}
\label{fig:algorithmOverview}
}
\end{figure*}
\fi






\iffalse
%-------- overview ---------
\textbf{Overview of the approach}. 
Our proposed network architecture (see Fig.~\ref{fig:algorithmOverview}) employs and adapts some of the architectural components recently proposed in~\cite{saha2017amtnet}.
% ---
At training time, the inputs to our deep network are a pair of successive RGB video frames~\textbf{(a.1)}~\cite{saha2017amtnet} and a set of five stacked optical flow maps~\textbf{(a.2)}~\cite{peng2016eccv} which are fed to an appearance~\textbf{(b.1)} and a motion stream~\textbf{(b.2)} respectively (\S~\ref{subsec:vgg16-fm-fusion}).
% ---
The appearance stream consists of two parallel CNNs and the motion stream is a single CNN network. The weights of these three CNNs are not shared among them and updated independently during training.
%---
The output feature maps of these three CNNs are fused~\textbf{(c)} and passed as input to a 3D region proposal network (3D-RPN)~\textbf{(d)}~(\S~\ref{subsec:3d-rpn}).
% ---
The 3D-RPN network generates 3D region proposals and their associated \emph{actionness}\footnote{The term \emph{actionness}~\cite{chen2014actionness} is used to denote the possibility of an action being present within a 3D region proposal.} \cite{chen2014actionness} scores, which are then sampled as positive and negative training examples by a 3D proposal sampler~\textbf{(d)}~(\S~\ref{subsec:prop-sampler}).
% ---
A training mini-batch of $B$ examples are constructed from these positive and negative 3D proposals, in this work we set $B=256$.
% ---
The mini-batch is firstly used to compute the \emph{actionness} classification and 3D proposal regression losses,
and secondly, to pool CNN features for each 3D proposal using a bilinear interpolation layer~\textbf{(e)}~(\S~\ref{bilinear-interpolation}).
The  bilinear interpolation gives rise to a fixed-size pooled feature map (for each 3D proposal) of size $[512 \times kh \times kw]$, where $kh$ $=$ $kw$ $=$ $7$.
% ---
Each pooled feature map (i.e., an spatio-temporal feature encoding of a 3D proposal)~\textbf{(e)} is passed to two fully connected layers (FC6 and FC7)~\textbf{(f)}~(\S~\ref{subsec:fc-layers}).
The output of the FC7 layer is a fixed sized feature vector of shape $[4096 \times 1]$.
These $4096$ dimension feature vectors are then used by a classification and a regression layers~\textbf{(f)}~(\S~\ref{subsec:fc-layers}) to output
\textbf{(1)} $B \times C$ classification scores and  
\textbf{(2)} $B \times C \times 8$ coordinate values where 
$B$ is the number of 3D proposals in a training mini-batch and $C$ is the number of action categories in a given dataset.
% ---
At test time we select top $300$ predicted micro-tubes by using non-maximum suppression, modified to work with pairs of bounding boxes
and pass these to an action-tube generator~\textbf{(g)}~(\S~\ref{sec:action-tube}) which links those micro-tubes in time.
At both training and test time, our model receives as input successive video frames $f_{t}$, $f_{t+\Delta}$. 
As we show in the Section~\ref{subsec:discussion}, even consecutive frames ($\Delta=1$) carry significantly different information which affects the overall video-mAP. % end
\fi

==> text/3_approach.old.tex <==


\section{AMTnet-Flow offline model} \label{sec:amtnet-flow-offline}
% All the components of the proposed deep network architecture (Fig.~\ref{fig:amtnet-flow-offline}) are described below in detail.
% \subsection{Convolutional neural network} 
% \label{ch:iccv2017:sec:net_arch:subsec:vgg16-fm-fusion}
% We adapt the network architecture of AMTnet~\cite{saha2017amtnet}. 

Fig.~\ref{fig:amtnet-flow-offline} illustrates the AMTnet-Flow offline action detection pipeline.
We add a motion stream (Fig.~\ref{fig:amtnet-flow-offline}~{(b.2)}) to the existing AMTnet architecture~\cite{saha2017amtnet} and introduce a RGB and optical flow feature fusion layer (Fig.~\ref{fig:amtnet-flow-offline}~{(c)}).
We follow VGG-16 network architecture~\cite{simonyan2014two} for our two appearance and one motion streams (Fig.~\ref{fig:amtnet-flow-offline}~{(b.1)}~\&~{(b.2)}).
We keep all the layers of VGG-16 from the first layer to the last ($13$-th) conv layer, and discard the remaining layers.
In this paper, we termed this modified VGG as VGG-16$^{*}$.
The weights are not shared among these three CNNs (2 for appearance and 1 for motion stream), and thus, during training they learn three different sets of weights.
Each VGG-16$^{*}$ has $13$ conv layers intermixed with $5$ max pooling layers.
Each conv layer has a $3 \times 3$ filter and $1 \times 1$ stride and padding.
Each max pooling layer has filter shape $2 \times 2$.
% We discard all the VGG-16 layers after the last ($13$-th) conv layer.

%-------------------------------------------
\subsection{Appearance streams}
We use two parallel VGG-16$^{*}$ for our appearance streams~(Fig.~\ref{fig:amtnet-flow-offline} (b.1)).
At each forward pass (during training and testing), these two CNNs receive two RGB video frames, each of which belongs to two different time points, i.e., they are successive frames
$f_t$ and $f_{t+\Delta}$~(Fig.~\ref{fig:amtnet-flow-offline} (a.1)).
% two successive RGB video frames $f_t$ and $f_{t+\Delta}$~(Fig.~\ref{fig:amtnet-flow-offline} (a.1)) and
The two parallel CNNs process them through $13$ conv layers (intermixed with $5$ max pooling layers) in parallel.
The output of each CNN is a conv feature map produced by the last conv layer which has dimension $[D \times H' \times W']$ where $D=512$, $H'=\frac{H}{16}$, and  $W'=\frac{W}{16}$, $H$ is the input frame height, $W$ is the frame width.

%-------------------------------------------
\subsection{Motion stream}
We use a single VGG-16$^{*}$ for the motion stream~(Fig.~\ref{fig:amtnet-flow-offline} (b.2)). 
The motion stream takes $5$ stacked optical flow maps~(Fig.~\ref{fig:amtnet-flow-offline} (a.2))~\cite{peng2016eccv} as input. 
It processes the stacked flow maps in parallel to the appearance streams, and outputs a feature map of dimension $[D \times H' \times W']$.
We refer the readers to the supplementary material for further details on motion stream implementation.
% Section~\ref{ch:bmvc2017:sec:imp_details:subsec:motion_cnn_arch_modification} 
% for  details.

%-------------------------------------------
\subsection{Conv feature map fusion} \label{sec:amtnet-flow-offline-featfusion}
The three conv feature maps of shape $[D \times H' \times W']$ (two from the appearance and one from the motion stream) are then fused using a element-wise sum fusion~\cite{Feichtenhofer_2016_CVPR} and the resultant feature-map (having the same dimension $[D \times H' \times W']$)~(Fig.~\ref{fig:amtnet-flow-offline} (c)) is passed as input to a 3D region proposal network (3D-RPN)~(Fig.~\ref{fig:amtnet-flow-offline}~(d)), and subsequently to a 3D proposal feature pooling layer~(Fig.~\ref{fig:amtnet-flow-offline}~(e)).

\iffalse
\begin{figure}[!ht]
{
\centering
\includegraphics[width=0.45\textwidth]{figures/intro/3d_prop_micro_tube.pdf}
\caption
{
\textbf{(a)}: 
% A CNN learns a video based action representation from a pair of successive frames $(f_t$, $f_{t+\Delta})$.
% To learn a video based CNN feature representation of human actions, we solve a video level regression problem in which a transformation is learnt (based on conv features) that can 
A 3D-RPN maps a 3D region proposal (in red) to a ground truth micro tube (in green). 
Note that, the learnt video based representation can encode the temporal relationships between the ``diving'' action regions (denoted by bounding boxes in green) in frames $f_t$ and $f_{t+\Delta}$.
\textbf{(b)}: temporal linking of detection micro-tubes at testtime.
}
\label{sec:intro:fig:3dp_mt}
}
\end{figure} 
\fi
\begin{figure*}[!ht]
{
\centering
\includegraphics[width=0.99\textwidth]{figures/methodology/amtnet-flow-online.pdf}
\caption{Amtnet-Flow online action detection model.}
\label{fig:amtnet-flow-online}
}
\end{figure*}


\begin{figure*}[h!]
  \centering
  \includegraphics[width=0.7\textwidth]{figures/methodology/micro-tube-gen-link}
  \caption[Action micro-tube generation by linear interpolation.]
  {
  \textbf{(a)} Action micro-tube generation by linear interpolation of coordinates of predicted bounding boxes.
 The blue circles denote the $8$ $(x,y)$ coordinate values of bounding boxes predicted by our network for a pair of successive test video frames.
 The first frame in the pair belongs to time $t=1$ and the seconds frame belongs to time $t=4$.
 We generate the coordinates of detection bounding boxes (pink circles) for intermediate frames (i.e. frame $2$ and $3$)
 by linear interpolation of the predicted coordinates.
 Thus, at test time, our model processes a pair of successive frames by skipping two intermediate frames (in this example frame 2 and 3)
 which substantially reduces the computing cost and time and speeds up the detection process.
 \textbf{(b)} Action tube generation by linking micro-tubes generated by \textbf{(a)}.
 Note that, for a video sequence with $T$ frames, our model needs to process only $T/2$ frames and
 the micro-tube linking algorithm requires to connect only $(T/2)-2$ frames.
  }
  \label{fig:box-intrpl_mt_linking}
\end{figure*}

\begin{figure*}[ht!]
  \centering
  \includegraphics[width=0.7\textwidth]{figures/methodology/box-interpolation}
  \caption
  {Generation of detection bounding boxes for intermediate frames using linear interpolation.
  }
  \label{fig:box-interpolation}
\end{figure*}


\subsection{3D region proposal network} \label{sec:offline:subsec:3drpn}
\label{ch:iccv2017:sec:net_arc:subsec:3d-rpn}
The 3D-RPN network~\cite{saha2017amtnet} (Fig.~\ref{fig:amtnet-flow-offline}~(d)) design is based on the basic principles of the 2D RPN network~\cite{ren2015faster}.
Unlike a 2D RPN which generates region proposals (rectangular bounding boxes) per image, the 3D-RPN network generates 3D region proposals spanning a pair of video frames (Fig.~\ref{sec:intro:fig:3dp_mt}~(a)).
A single 3D proposal thus consists of a pair of rectangular bounding boxes.
The input to the 3D-RPN is a fused VGG-16 feature map~(Fig.~\ref{fig:amtnet-flow-offline}~(c)) of size $[512 \times H' \times W']$.
It generates anchor boxes in a similar way as in~\cite{ren2015faster}: namely, it projects back each point in the $H' \times W'$ grid (of the input feature map) onto the original image plane of size $H \times W$.
For each projected point, the 3D-RPN generates $k$ pairs of anchor boxes of different aspect ratios.
Due to a large number of 3D region proposals (e.g., for k=12, we have $k \times H' \times W' = 12 \times 38 \times 50 = 22800$ proposals), they are subsampled (Fig.~\ref{fig:amtnet-flow-offline}~(d)).
During training, those proposals which have mean IoU $\geq 0.5$ with the ground truth micro-tube (Fig.~\ref{sec:intro:fig:3dp_mt}~(a)) are considered as positive,
and those having mean IoU $< 0.3$ are negatives. The RPN's binary classification (i.e. action or background) and 3D proposal regression losses are computed based on $B$ such top positive and negative training examples where, $B$ is the training mini-batch size and we set it to $256$.
Thus, the 3D-RPN gives us $P$ positive and $B-P$ negative examples (i.e. 3D proposals) to train the AMTnet-Flow network.
During testing, we use non-maximum suppression (NMS) to select the top $2000$ proposals.

% TODO maybe you can put in the appendix -- but not required - 3D RPN anyway not a contribution of this paper and it is contribution of AMTnet paper -- people will refer amtnet paper if they want details on it
\iffalse
\label{ch:iccv2017:sec:net_arch}
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/methodology/3d-rpn.pdf}
  \caption[3D-RPN  architecture.]
  {
  3D-RPN  architecture.
  }
  \label{ch:iccv2017:sec:net_arch:fig:3d-rpn}
\end{figure*}

The network architecture of the 3D-RPN is depicted in~Figure~\ref{ch:iccv2017:sec:net_arch:fig:3d-rpn}.
To encode the location information of each pair of anchors, we pass the fused VGG-16 feature map through a $3 \times 3$ convolution~\textbf{(b)}, a rectified linear nonlinearity~\textbf{(c)}, and two more $1 \times 1$ convolution~(\textbf{(e)} and~\textbf{(h)}) layers. 
The first conv layer~\textbf{(b)} consists of 256 convolution filters with $1 \times 1$ stride and padding, resulting in a feature map of size $[256 \times H' \times W']$~\textbf{(d)}.  
The second conv layer~\textbf{(e)} has $8 \times k$ convolution filters with $1 \times 1$ stride and does not have padding.
It outputs a feature map of shape $[(8 \times k) \times H' \times W']$~\textbf{(f)} which encodes the location information (8 coordinate values) of $[ k \times H' \times W']$ pairs of anchor boxes~\textbf{(g)}.
The third conv layer~\textbf{(h)} is the same as~\textbf{(e)}. The only difference is in the 
number of filters which is $2 \times k$ to encode the actionness score (i.e. probability of action or no-action) ~\textbf{(j)} for each $k$ pairs of anchors.
% As RPN is a fully convolutional neural network, classification and regression weights are learned directly from the convolution features, whereas in the fully connected layers we apply linear transformation layers for classification and regression.
In the 3D-RPN, the convolution layer~\textbf{(e)} is considered as the regression layer, as it outputs the 8 regression offsets per pair of anchor boxes; the convolution layer~\textbf{(h)} is the classification layer.
\fi

%-------------------------------------------


%-------------------------------------------
\subsection{3D proposal feature pooling}
We pool CNN features for these $B$  (i.e. 256) training examples using \emph{bilinear interpolation}~\cite{gregor2015draw,jaderberg2015spatial}~(Fig.~\ref{fig:amtnet-flow-offline}~(e)).
The output of the feature pooling step is a fixed sized feature vector (of shape $[D \times kh \times kw]$, where $D=512$, $kh=kw=7$) for each 3D proposal, we have such $B$ feature vectors which are passed as inputs to the FC6 layer~(Fig.~\ref{fig:amtnet-flow-offline}~(f)) for training a multi-class classifier and a 3D proposal regressor.  


%-------------------------------------------
\subsection{Fully connected, classification and regression layers}
A mini-batch of $B$ (i.e. 256) pooled conv feature vectors (of $B$ positive and negative examples) are passed through a FC6, FC7, classification and regression layers~(Fig.~\ref{fig:amtnet-flow-offline}~(f)).
The final outputs of the network at train time are:
(1) $B \times C$ action classification scores and
(2) $B \times C \times 8$ micro-tube regression offsets for $B$ training examples.
The network's final action classification and micro-tube regression losses are computed based on the these network outputs. 

%-------------------------------------------
\subsection{Offline action tube generation} \label{sec:amtnet-flow-offline-tubegen}
At test time, we select top $300$ detection micro-tubes using NMS and then apply our offline micro-tube linking algorithm to build the final action tubes.
We adapt the micro-tube linking algorithm of~\cite{saha2017amtnet} and modified it to link relatively longer micro-tubes (i.e. $\Delta=3$ (ours) instead $\Delta=1$ of ~\cite{saha2017amtnet}).



\section{AMTnet-Flow online model} \label{sec:amtnet-flow-online}

Fig.~\ref{fig:amtnet-flow-online} illustrates the AMTnet-Flow online action detection pipeline.
We replace the Faster-RCNN network architecture~\cite{ren2015faster} in the AMTnet-Flow offline model (Section~\ref{sec:amtnet-flow-offline}) with relatively faster and efficient SSD network~\cite{liu2016ssd}.
An SSD network consists of a VGG-16* base network followed by two conv layers (i.e., Conv6 and Conv7 which are the replacements for the FC6 and FC7 layers in Faster-RCNN) and $4$ extra conv layers (i.e. Conv8-2, Conv9-2, Conv10-2 and Conv11-2).
These conv layers, VGG-16*'s Conv4-3, Conv7 and these $4$ additional conv layers have decreasing output dimensions,
i.e., they output feature maps having shape in a decreasing order. 
For example, Conv4-3 has output feature map dimension $38 \times 38$, Conv7 has $19 \times 19$, Conv8-2 has $10 \times 10$ and so on. 
Thus, SSD learns representation from feature maps at different scales,
the largest dimension $18 \times 18$ represents the smallest 2D spatial scale, whereas the the smallest $1 \times 1$ represents the largest scale.


% with decreasing size to have feature representation along different scales.


% Similarly as in AMTnet-Flow offline model, here we use VGG-16* as a base network (i.e. default in SSD) for the three streams (2 appearance streams and 1 motion stream) and the weights are not shared among them.

\subsection{Appearance streams}
We use two parallel SSD networks as the appearance streams (Fig.~\ref{fig:amtnet-flow-online} (b.1)).
At each forward pass (during both training and testing), these two appearance streams receive as input two RGB video frames, each of which belongs to two different time points, i.e., they are successive frames $f_t$ and $f_{t+\Delta}$~(Fig.~\ref{fig:amtnet-flow-online} (a.1)).
These RGB frames are pre-processed using SSD's data augmentation module before passing them to the appearance streams.
We apply exactly the same sets of augmentation to both the frames.
The two parallel appearance streams propagate these RGB frames through several conv layers which output feature maps at different spatial scales.

%--------------------------
\subsection{Motion stream}
We use a single SSD network as the motion stream (Fig.~\ref{fig:amtnet-flow-online} (b.2)).
The motion stream takes $5$ stacked optical flow maps~(Fig.~\ref{fig:amtnet-flow-online} (a.2))~\cite{peng2016eccv} as input. 
It processes the stacked flow maps in parallel to the appearance streams, and outputs conv feature maps at different spatial scales similar to the appearance streams.
We refer the readers to the supplementary material for further details on motion stream implementation.
% We refer the readers to Section~\ref{ch:bmvc2017:sec:imp_details:subsec:motion_cnn_arch_modification} for motion stream implementation details.


%-------------------------------------------
\subsection{Conv feature map fusion} \label{sec:amtnet-flow-online-featfusion}
The output conv feature maps dimensions for these three streams (2 appearance, 1 motion) are same at each feautre map's spatial scales and they are as follows:
$[512 \times 38 \times 38]$, $[1024 \times 19 \times 19]$, $[512 \times 10 \times 10]$, $[256 \times 5 \times 5]$, $[256 \times 3 \times 3]$ and $[256 \times 1 \times 1]$. 
At each spatial scale, the three conv feature maps (2 from the appearance streams and 1 from the motion stream) are fused using an element-wise sum fusion~(Fig.~\ref{fig:amtnet-flow-online} (c)) and the resultant fused feature maps~(Fig.~\ref{fig:amtnet-flow-online} (d)) are the final outputs of the network~(Fig.~\ref{fig:amtnet-flow-online} (e)), i.e., $8732$ detection micro-tubes' $8$ location offsets and $C$ softmax classifcation scores.
We apply NMS ~(Fig.~\ref{fig:amtnet-flow-online} (f)) to select the top $k$ micro-tubes to finally build the action tubes in an online fashion~(Fig.~\ref{fig:amtnet-flow-online} (g)).

\subsection{Online action tube generation} \label{sec:online:subsec:tubegen}
% \textcolor{red}{Gurkirt could you please write a para or two for the online tube gen algorithm referring your ICCV2017 paper.}
\SAHA{Gurkirt could you please write a para or two for the online tube gen algorithm.}

%---------------------------------------------------

\section{Bounding box interpolation} 
\label{sec:box_interpolation}
At test time, for a input pair of successive video frames ($f_{t}$ and $f_{t+\Delta}$), the final outputs of AMTnet-Flow (both offline and online models) are the top $k$ detection micro-tubes and their softmax classification scores.
For example, in Figure~\ref{fig:box-intrpl_mt_linking}~(a), we can visualise that for an input pair $(F1,F4)$ our network predicts an action micro-tube (depicted by the 2 blue bounding boxes) with 8 coordinate values (blue circles). In practice, the network predicts such 300 micro-tubes for an input pair.
Note that, yet we do not have detection bounding boxes for intermediate frames, in this example those are frames $F2$ and $F3$. 
We generate the detection boxes for the intermediate frames using a simple but elegant box interpolation algorithm which is explained in the next section.

As depicted in Figure~\ref{fig:box-interpolation}, the $8$ predicted bounding box coordinates $[(x_1,y_1,x_2,y_2)^{t_{1}}]$ and $[(x_1,y_1,x_2,y_2)^{t_{4}}]$ (shown in blue) which are known, and we would like to infer the unknowns $[(x_1,y_1,x_2,y_2)^{t_{2}}]$ and $[(x_1,y_1,x_2,y_2)^{t_{3}}]$ (shown in pink).
Using simple linear interpolation we can compute the unknowns using the following equation:
\begin{align} 
% \label{eqn:box-interpolation_1}
x_{1}^{t2} &=  x_{1}^{t1}(1-\frac{t_2-t_1}{t_4-t_1})+x_{1}^{t4}(1-\frac{t_2-t_1}{t_4-t_1}) \\ 
y_{1}^{t2} &=  y_{1}^{t1}(1-\frac{t_2-t_1}{t_4-t_1})+y_{1}^{t4}(1-\frac{t_2-t_1}{t_4-t_1}) \\
x_{1}^{t3} &=  x_{1}^{t1}(1-\frac{t_3-t_1}{t_4-t_1})+x_{1}^{t4}(1-\frac{t_3-t_1}{t_4-t_1}) \\ 
y_{1}^{t3} &=  y_{1}^{t1}(1-\frac{t_3-t_1}{t_4-t_1})+y_{1}^{t4}(1-\frac{t_3-t_1}{t_4-t_1}) 
\end{align}
Similarly we can compute $(x_2,y_2)^{t2}$ and $(x_2,y_2)^{t3}$.

%------------------------------------

\section{Action tube generation}
\label{ch:bmvc2017:sec:bbiatg:subsec:tube_gen}
Once the bounding-boxes for intermediate frames are generated using a linear interpolation algorithm (Section~\ref{sec:box_interpolation}) for each micro-tube, we can then temporally link them (Figure~\ref{fig:box-intrpl_mt_linking} (b)) using action tube generation algorithm of Saha~\etal~\cite{saha2017amtnet} for the offline and Singh~\etal~\cite{singh2016online} for the online model.
Unlike in~\cite{saha2017amtnet} in which micro-tubes are extracted for consecutive frame pairs  (i.e. $\Delta=1$), we use long distance frame pairs at test time.
For example, when $\Delta=3$, our micro-tube linking algorithm iterates only $(T/4-1)$ times to link all the micro-tubes associated with an action instance within a video.
Thus, our tube generation algorithm is relatively faster and requires less computing time and resources than the one in~\cite{saha2017amtnet}.
Figure~\ref{fig:box-intrpl_mt_linking}~(b) illustrates the efficacy of our micro-tube linking algorithm, i.e., our algorithm requires only $3$ iterations to link the micro-tubes of a video having $16$ frames, whereas ~\cite{saha2017amtnet}'s algorithm needs $7$ iterations.


%-------------------------------------


==> text/4_exp.old.tex <==
\section{Experiments} \label{sec:experiment}

\subsection{Datasets and evaluation metrics} 
We select the following two standard benchmarks to evaluate our proposed action detection approach.

\textbf{J-HMDB-21}~\cite{J-HMDB-Jhuang-2013} is a spatial action detection dataset (i.e. videos are temporally trimmed as per the action duration) comprises of $928$ video clips and $21$ action categories with $3$ train and test splits.
We report our evaluation results averaged over the $3$ splits.

\textbf{UCF-101-24}~\cite{soomro-2012} is a spatiotemporal action detection dataset which is a subset of the UCF-101 action recognition dataset.
It consists of $3207$ videos and $24$ action classes.
We report our evaluation results on the $1^{st}$ split of UCF-101-24.
Ground-truth bounding boxes for human silhouettes are provided for both the above datasets.

\begin{table*}[t]
  %\vskip -3mm
  \centering
  \setlength{\tabcolsep}{4pt}
  \caption{Action localisation results on JHMDB dataset.
  The table is divided into four parts. 
  The first part lists approaches which takes a single frame as input;
  the second part presents approaches which takes multiple frames as input;
  the third part contemplates different fusion strategies of our feature-level 
  fusion (based on AMTnet);
  lastly, we report the detection performance of our TPnet by ignoring the future and past predictions and only use the detected micro-tubes to produce the final action tubes.}
  \vspace{-2mm}
  {\footnotesize
  \scalebox{1}{
  \begin{tabular}{lccccc}
  \toprule
  Methods & $\delta$ = 0.2 &$\delta$ = 0.5 & $\delta$ = 0.75 & $\delta$ = .5:.95 & Acc \%\\\midrule
  MR-TS Peng~\etal cite{peng2016eccv} & 74.1  & 73.1 & -- & -- & --\\
  FasterRCNN Saha~\etal cite{Saha2016}   & 72.2  & 71.5 & 43.5 & 40.0 & --\\
  OJLA Behl~\etal cite{behl2017incremental}${}^*$  & -- & 67.3 & -- & 36.1 & --\\
  SSD Singh~\etal cite{singh2016online}${}^*$  & 73.8 & 72.0 & 44.5 & 41.6 & --\\
  \midrule
  AMTnet Saha~\etal cite{saha2017amtnet} rgb-only  & 57.7  & 55.3 & -- & -- & --\\
  ACT kalogeiton~\etal cite{kalogeiton2017action}${}^*$   & 74.2 & 73.7 & 52.1 & 44.8 & 61.7 \\
  T-CNN (offline) Hou~\etal cite{hou2017tube} & \textbf{78.4} & 76.9   & -- & -- & 67.2 \\
  %MR-TS~\cite{peng2016eccv} + I3D~\cite{carreira2017quo} Gu \etal~\cite{ava2017gu}  
  %& --  & \textbf{78.6} & -- & -- & --\\
  \midrule
  AMTnet-LateFusion${}^*$  & 71.7 & 71.2 & 49.7 & 42.5 & 65.8 \\
  AMTnet-FeatFusion-Concat${}^*$  & 73.1 & 72.6 & 59.8 & 48.3 & 68.4 \\
  AMTnet-FeatFusion-Sum${}^*$  & 73.5 & 72.8 & 59.7 & 48.1 & 69.6 \\
  \bottomrule
  % \vskip{2mm}
  \multicolumn{6}{l}{ ${}^*$ means online methods}\\
  \end{tabular}
  }
  }
  \label{table:localisationJHMDB21} %\vspace{-6mm}
\end{table*}

\begin{table*}[t]
  %\vskip -3mm
  \centering
  \setlength{\tabcolsep}{4pt}
  \caption{Action localisation results on JHMDB dataset.
  The table is divided into four parts. 
  The first part lists approaches which takes a single frame as input;
  the second part presents approaches which takes multiple frames as input;
  the third part contemplates different fusion strategies of our feature-level 
  fusion (based on AMTnet);
  lastly, we report the detection performance of our TPnet by ignoring the future and past predictions and only use the detected micro-tubes to produce the final action tubes.}
  \vspace{-2mm}
  {\footnotesize
  \scalebox{1}{
  \begin{tabular}{lccccc}
  \toprule
  Methods & $\delta$ = 0.2 &$\delta$ = 0.5 & $\delta$ = 0.75 & $\delta$ = .5:.95 & Acc \%\\\midrule
  MR-TS Peng~\etal cite{peng2016eccv} & 73.7  & 32.1 & 00.9 & 07.3 & --\\
  FasterRCNN Saha~\etal cite{Saha2016}   & 66.6  & 36.4 & 07.9 & 14.4 & --\\
  OJLA Behl~\etal cite{behl2017incremental}${}^*$  & -- & -- & -- & -- & --\\
  SSD Singh~\etal cite{singh2016online}${}^*$  & 76.4 & 45.2 & 14.4 & 20.1 & 92.2 \\
  \midrule
  AMTnet Saha~\etal cite{saha2017amtnet} rgb-only  & --  & -- & -- & -- & --\\
  ACT kalogeiton~\etal cite{kalogeiton2017action}${}^*$   & 76.5 & 49.2 & 19.7 & 23.4 & -- \\
  T-CNN (offline) Hou~\etal cite{hou2017tube} & -- & --   & -- & -- & -- \\
  %MR-TS~\cite{peng2016eccv} + I3D~\cite{carreira2017quo} Gu \etal~\cite{ava2017gu}  
  %& --  & \textbf{78.6} & -- & -- & --\\
  \midrule
  AMTnet rgb-only  & 75.8 & 45.3 & 19.9 & 22.0  & 90.0 \\
  AMTnet flow-only  & 73.7 & 41.6 & 11.3 & 17.1  & 87.8 \\
  AMTnet-LateFusion${}^*$  & 79.7 & 49.1 & 19.8 & 22.9  & 92.3 \\
  AMTnet-FeatFusion-Concat${}^*$  & 79.2 & 49.0 & 21.4 & 24.1  & 90.7 \\
  AMTnet-FeatFusion-Sum${}^*$  & 79.4 & 50.7 & 21.8 & 24.5  & 91.5 \\
  \bottomrule
  % \vskip{2mm}
  \multicolumn{6}{l}{ ${}^*$ means online methods}\\
  \end{tabular}
  }
  }
  \label{table:localisationUCF24} %\vspace{-6mm}
\end{table*}

%-------------------------------------------------------------------------------------------------
\begin{table*}[!t] 
\caption{Impact of adding motion stream on action detection performance, J-HMDB-21 (*) dataset.} 
\label{table:eff_motion_stream}
\centering
\scalebox{0.99}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c}{Video-mAP} & \multicolumn{1}{c}{Frame-mAP} \\
$\delta$ & 0.1 & 0.2 & 0.3 & 0.4 & 0.5     & 0.5   \\ \midrule
AMTnet & 57.79 & 57.76 & 57.68 & 56.79 & 55.31     & 45.0   \\
AMTnet-Flow offline & \textbf{64.64} & \textbf{64.64} & \textbf{64.57} & \textbf{64.01} & \textbf{62.68} & \textbf{52.08}   \\  \\
\multicolumn{7}{l}{(*)Trained \emph{model-11+32}, action tubes generated using micro-tube linking algorithm as in~\cite{saha2017amtnet}. } \\ 
\bottomrule 
\end{tabular}
}
\end{table*} 

%----------------------------

\begin{table*}[t!] 
\centering
\footnotesize
\caption{Impact of adding motion stream on action detection performance, UCF-101-24 (*) dataset.} 
\scalebox{0.95}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c}{Video-mAP} & \multicolumn{1}{c}{Frame-mAP} \\
$\delta$ & 0.1 & 0.2 & 0.3 & 0.4 & 0.5                     & 0.5 \\   \midrule
AMTnet & 71.3 & 63.06 & 51.57 & 43.10 & 33.06            & 54.91  \\
AMTnet-Flow offline & \textbf{79.65} & \textbf{71.51} & \textbf{59.79} & \textbf{47.28} & \textbf{35.77} & \textbf{62.70}  \\  \\

\multicolumn{7}{l}{(*)Trained \emph{model-21}, action tubes generated using 2PDP with cross validated alphas as in~\cite{Saha2016}.} \\
\bottomrule 
\end{tabular}
}
\label{table:eff_motion_stream_ucf101}
\end{table*}
%----------------------------

\begin{table}[t!] 
\centering
\footnotesize
\caption{
Impact of bounding box interpolation on action detection performance (video-mAP).
} 
\scalebox{0.95}{
\begin{tabular}{l|ccc|ccc}
\toprule
% \multicolumn{1}{c}{}       & \multicolumn{6}{c}{Detection performance (video-mAP)}  \\ 
\multicolumn{1}{c|}{}       & \multicolumn{3}{c|}{J-HMDB} & \multicolumn{3}{c}{UCF-101}  \\ 
$\delta$                    & 0.2           & 0.4            & 0.5                   & 0.2               & 0.5               & 0.5:0.95 \\ \midrule
w/o interpolation           & \textbf{64.73} & \textbf{64.32} & \textbf{62.67}       & \textbf{71.57}    & 35.77             & 10.9   \\ 
with interpolation          & 64.63         & 64.27          & 61.97                 & 69.86             & \textbf{37.15}    & \textbf{11.9} \\ 
 \bottomrule
\end{tabular}
}
\label{table:eff_box_interpolation}
\end{table} 

%----------------------------

\begin{table}[t!] 
\centering
\footnotesize
\caption{
Impact of bounding box interpolation on action detection speed (seconds / video).
} 
\scalebox{0.95}{
\begin{tabular}{l|cc}
\toprule
\multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{J-HMDB} & \multicolumn{1}{c}{UCF-101} \\  \midrule
w/o interpolation           & 11.9 & 61.25 \\ 
with interpolation          & \textbf{5.95} & \textbf{30.62} \\ 
\bottomrule
\end{tabular}
}
\label{table:eff_box_interpolation_speed}
\end{table}

\begin{table}[t] 
\centering
\footnotesize
\caption{
Impact of our action tube generation algorithm on compute time (in seconds per video).
}
\scalebox{0.85}{
\begin{tabular}{ccc|ccc}
\toprule
-- &  Saha~\etal~\cite{Saha2016} & Ours & -- &  Saha~\etal~\cite{Saha2016} & Ours \\ \midrule
J-HMDB-21 & 0.38 & \textbf{0.16} & UCF-101-24 & 0.96 & \textbf{0.47} \\
 \bottomrule
\end{tabular}
}
\label{table:action-tube-compute-time}
\end{table} 

%----------------------soa ----------------------
\begin{table}[t!] 
\centering
\footnotesize
\caption{
Comparison with the state-of-art on J-HMDB-21 dataset.
} 
\scalebox{0.95}{
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Video-mAP}   & \multicolumn{1}{c}{Frame-mAP} \\ 
%\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{J-HMDB}      & \multicolumn{5}{c|}{UCF-101} & \multicolumn{1}{c|}{J-HMDB}   & \multicolumn{1}{c}{UCF-101}   \\ \midrule
 $\delta$                                      & 0.2               & 0.5     & 0.5    \\ \midrule
 Gkioxari~\etal~\cite{Georgia-2015a}           & --                & 53.3                       & 36.2      \\
 Wang \etal~\cite{wangcvpr2016}                & --                & 56.4                       & 39.9       \\
 Weinzaepfel~\etal~\cite{Weinzaepfel-2015}     & --                & 60.7                       & 45.8   \\
 Yu~\etal~\cite{yu2015fast}                    & --                & --                         & --  \\
 Saha~\etal~\cite{Saha2016}                    & 72.63             & 71.50                      & --  \\
 Saha~\etal~\cite{saha2017amtnet}              & 57.76             & 55.31                      & 45.0 \\
 Peng~\etal~\cite{peng2016eccv}                & \textbf{74.3}     & \textbf{73.1}              & \textbf{58.5}  \\
 Ours (w/o interpolation)                      & 64.73             & 62.67                      & 52.08 \\ 
 Ours (with interpolation)                     & 64.63             & 61.97                      & 52.73 \\ 
 \bottomrule
\end{tabular}
}
\label{table:com-soa-jhmdb21}
\end{table} 


\begin{table}[t!] 
\centering
\footnotesize
\caption{
Comparison with the state-of-art on UCF-101-24 dataset.
} 
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{Video-mAP}   & \multicolumn{1}{c}{Frame-mAP} \\ 
%\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{J-HMDB}      & \multicolumn{5}{c|}{UCF-101} & \multicolumn{1}{c|}{J-HMDB}   & \multicolumn{1}{c}{UCF-101}   \\ \midrule
 $\delta$                                      & 0.1                   & 0.2                                    & 0.5               & 0.5:0.95                   & 0.5 \\ \midrule
 Gkioxari~\etal~\cite{Georgia-2015a}           & --                    & --                                     & --                & --                          & --\\
 Wang \etal~\cite{wangcvpr2016}                & --                    & --                                     & --                & --                         & --\\
 Weinzaepfel~\etal~\cite{Weinzaepfel-2015}     & 51.7                  & 46.8                                   & --                & --                         & 35.84 \\
 Yu~\etal~\cite{yu2015fast}                    & 42.8                  & 26.5                                   & --                & --                         & -- \\
 Saha~\etal~\cite{Saha2016}                    & 76.12                 & 66.36                                  & 34.82             & --                         & --\\
 Saha~\etal~\cite{saha2017amtnet}              & 71.3                  & 63.06                                  & 33.06             & 10.72                      & 54.91\\
 Peng~\etal~\cite{peng2016eccv}                & 77.31                 & \textbf{72.86}                         & 30.87             & 07.11                      &\textbf{65.73} \\
 Ours (w/o interpolation)                      & \textbf{79.65}        & 71.57                                  & 35.77             & 10.96                      & 62.7\\ 
 Ours (with interpolation)                     & 78.24                 & 69.86                                  & \textbf{37.15}    & \textbf{11.9}              & 62.86 \\ 
 \bottomrule
\end{tabular}
}
\label{table:com-soa-ucf101}
\end{table}
%-------------------------------------------------------------------------------------------------


\textbf{Evaluation metrics.} We use the standard \emph{frame-mAP}~\cite{Georgia-2015a,peng2016eccv} and \emph{video-mAP}~\cite{Georgia-2015a,Weinzaepfel-2015,Saha2016,peng2016eccv} (mean average precision).
For video-mAP evaluation, we select the IoU threshold ($\delta$) range $[0.1:0.1:0.5]$.
For UCF-101-24, we compute the video-mAPs at higher IoU threshold range between $[0.5:0.05:0.95]$, and then we compute the mean video-mAP which we denote as $(0.5:0.95)$.
For frame-mAP we set IoU threshold $\delta=0.5$ for both J-HMDB-21 and UCF-101-24. 




\subsection{AMTnet-Flow offline model evaluation}

\subsubsection{Experimental settings} 
We follow the training data sampling strategy as in~\cite{saha2017amtnet}, in addition, for training on long distance pairs we introduce a new scheme \emph{scheme-43}.
Throughout this section we use the following naming conventions to denote models trained on training sets generated using different sampling strategies:
a) a model trained on training data generated using \emph{scheme-11} and \emph{-32}~\cite{saha2017amtnet} is referred as \emph{model-11+32};
b) \emph{model-11+32+43} refers to the model trained using \emph{scheme-11}, \emph{-32} and \emph{-43};
similarly, c) \emph{model-21} and d) \emph{model-21+43}.
For more details on the train and test data sampling schemes, implementation details please refer the supplementary material.

\subsubsection{Impact of adding motion stream} \label{sec:exp:subsec:offline:motstream}
We observe a significant improvement in action detection performance by adding an extra flow stream to the AMTnet architecture.
For this experiment, we first reproduce the results of AMTnet~\cite{saha2017amtnet} on both J-HMDB-21 and UCF-101-24 datasets following their train and test time settings.
Then, we introduce our motion-stream alongside the two spatial streams of AMTnet, and train the model on both the datasets following AMTnet's train and test time settings.
In Table~\ref{table:eff_motion_stream} and \ref{table:eff_motion_stream_ucf101}, we refer these models as AMTnet and AMTnet-Flow offline where the video- and frame-mAPs at different IoU thresholds ($\delta$) for these two models are shown.
Note that for J-HMDB, the video- and frame-mAP are improved by \textbf{7.37\%} and \textbf{7.08\%} at $\delta=0.5$ (Table~\ref{table:eff_motion_stream}).
For UCF-101-24, video-mAP (at $\delta=0.2$) and frame-mAP (at $\delta=0.5$) are improved by\textbf{8.45\%} and \textbf{7.79\%} (Table~\ref{table:eff_motion_stream_ucf101}).



\subsubsection{Impact of bounding box interpolation on performance and speed} 
\label{sec:exp:subsec:offline:subsub:boxinterpol}
For this experiment, we train our model on J-HMDB-21 and UCF-101-24 datasets on both short and long distance pairs.
% TODO -- we need to copy the text from my thesis Section~\ref{ch:bmvc2017:sec:train_data_sampl_scheme} to supplementary material
In the supplementary material we discuss in detail the different training data sampling schemes used to generate the training data for each model in this experiment.
At test time, we generate two sets of detection results to demonstrate the efficacy of our bounding box interpolation algorithm (Section~\ref{sec:box_interpolation}).
First set of micro-tubes are extracted by passing test pairs $f_t$ and $f_{t+\Delta}$ where $\Delta=1$ (short distance pairs).
Second set of micro-tubes are extracted by passing test pairs where $\Delta=3$ (long distance pairs).
For micro-tubes extracted using long-distance pairs, we fill in the  intermediate frames' bounding boxes using our box interpolation algorithm (Section~\ref{sec:box_interpolation}).
We denote these two sets of results in Table~\ref{table:eff_box_interpolation}  and Table~\ref{table:eff_box_interpolation_speed} as ``w/o interpolation'' and ``with interpolation''.
Our bounding box interpolation algorithm improves the test time detection speed significantly without affecting the detection performance (Table~\ref{table:eff_box_interpolation_speed}).
For J-HMDB-21, it improves the detection speed from $11.9$ sec/vid (seconds per video) to \textbf{5.95} sec/vid, and for UCF-101, from $61.25$ sec/vid to \textbf{30.62} sec/vid.
Here detection speed denotes the compute time required for micro-tube extraction.
Interestingly, for UCF-101, it improves the video-mAP at higher thresholds, i.e., we observe a gain in the mAP by \textbf{1.38\%} and \textbf{1.0\%} at $\delta=0.5$ and $0.5:0.95$ respectively
(Table~\ref{table:eff_box_interpolation}).
Note that, the test video clips in UCF-101-24 have relatively longer duration (on average 175 frames) than J-HMDB-21 (on average 25 frames).
The relatively shorter test video clips might be the reason that our bounding box interpolation algorithm could not exhibit performance boost on J-HMDB-21.
We believe that, it will work gracefully for even longer sequences of videos where spatial locations of actions do not vary rapidly within shorter time span (e.g. within 5 or 10 frames).


\subsubsection{Impact of tube generation algorithm on compute time} 
\label{sec:exp:subsec:offline:subsub:tubegen}
To evaluate our modified offline action tube generation method (Section~\ref{ch:bmvc2017:sec:bbiatg:subsec:tube_gen}), we compare the detection performance and compute time requirement of our algorithm with~\cite{Saha2016}.
In Table~\ref{table:eff_box_interpolation}, the ``w/o interpolation'' refers to the results obtained using the action-tube generation algorithm~\cite{Saha2016}, and ``with interpolation'' denotes the results generated by our tube building approach.
Remarkably, with relatively lesser number of iterations $(T/4-1)$ as compared to $(T-1)$ iterations required by~\cite{Saha2016}, our action tube generation algorithm improves the video-mAP at higher thresholds on UCF-101.
Moreover, our method exhibits excellent mean detection speed (Table~\ref{table:action-tube-compute-time}) of $0.16$ sec/vid and $0.47$ sec/vid for J-HMDB and UCF-101 respectively.
In particular, it improves the speed by \textbf{0.22} (for J-HMDB) and \textbf{0.49} (for UCF-101) sec/vid over~\cite{Saha2016}'s approach.

\subsubsection{Comparison with the state-of-art}
In this section, we compare the action detection performance of the proposed approach with the state-of-the-art methods (see Table~\ref{table:com-soa-jhmdb21} and Table~\ref{table:com-soa-ucf101}).
The proposed approach outperforms the state-of-the-art methods~\cite{Georgia-2015a,wangcvpr2016,Weinzaepfel-2015,yu2015fast,saha2017amtnet} in both frame- and video-mAP on two benchmark datasets.
In addition, our approach outperforms the two close competitors~\cite{Saha2016,peng2016eccv} in spatio-temporal detection (video-mAP) on UCF-101.
More specifically,  it outperforms~\cite{Saha2016} (in video-mAP for UCF-101) by $5.21\%$ and $2.33\%$ at IoU threshold ($\delta$) values $0.2$ and $0.5$ respectively.
Although, on lower $\delta$ values ($0.2$ and $0.3$) our approach shows comparable results to~\cite{peng2016eccv}, on higher $\delta$s ($0.5$ and $0.5:0.95$), it achieves superior performance with a gain in the video-mAP by \textbf{6.28\%} and \textbf{4.79\%} respectively.

\iffalse
A lower detection performance of our approach on J-HMDB-21 as compared to~\cite{Saha2016,peng2016eccv} is due to the fact that J-HMDB is relatively smaller dataset and our network has large number of model parameters than~\cite{Saha2016,peng2016eccv} which might cause overfitting. 
In Section~\ref{ch:bmvc2017:sec:eval:subsec:comp_frame_video_aps}, we present the class-specific frame- and video-mAP comparison with the state-of-art.
\fi

\subsubsection{Discussion}
For some instances, Peng~\etal's~\cite{peng2016eccv} approach exhibits better detection performance  on UCF-101-24 than the proposed solution (Table~\ref{table:com-soa-ucf101}).
However, we argue that their approach is expensive.
Firstly, they train two separate networks for appearance and motion streams independently, they name their network as \emph{``two-stream R-CNNs''}.
Secondly, they finetune these two networks on \emph{multi-region} based action proposals using the learned weights of the two-stream R-CNNs (for more detail, please refer to~\cite{peng2016eccv}).
Note that, their framework follows a \emph{multi-stage} training strategy.
Moreover, they follow \emph{multi-scale} training and testing schemes in which at train (or test) time, for each original video frame three re-scaled versions of that frame are generated, and subsequently they are used for training or testing.
It is quite apparent that Peng~\etal's approach is computationally expensive both at training and testing.

In contrast, we train both the appearance and motion streams jointly and the proposed approach follows a \emph{single-stage} training i.e. our network requires only one time training and does not require any finetuning as in~\cite{peng2016eccv}.
At test time, the network receives a pair of successive video frames ($f_t$ and $f_{t+\Delta}$ where $\Delta=4$, see Figure~\ref{fig:box-intrpl_mt_linking} (a)) as input, and predicts pairs of bounding boxes (called action micro-tubes~\cite{saha2017amtnet}, see Figure~\ref{fig:box-intrpl_mt_linking} (b)) which are linked in time. 
Thus, our model requires to process only $50\%$ of the entire video frames which significantly reduces the computing time and cost.
Moreover, we follow single-scale training and testing schemes i.e., we use each video frame only once as compared to~\cite{peng2016eccv} which uses one frame thrice (at 3 different scales).
With these aforementioned properties i.e., an end-to-end trainable network and relatively low computing requirements, the proposed approach outperforms~\cite{peng2016eccv} at higher IoU thresholds ($\delta$) (Table~\ref{table:com-soa-ucf101}) on one of the largest action detection datasets (UCF-101-24~\cite{soomro-2012}) to date.


One of the standard techniques for reducing overfitting is data augmentation.
As discussed above, Peng~\etal~\cite{peng2016eccv} augment their training data with three re-scaled versions of the original video frame (i.e. the multi-scale training), and use three extra sets of region proposals alongside the original set of RPN proposals (i.e. the multi-region based action proposals). 
To train their network on these additional proposals, they add three extra ROI pooling layers (alongside the original RPN-based ROI pooling layer).
Although, their multi-scale and multi-region based training approach helps in improving the detection performance on J-HMDB-21, they are expensive.
As J-HMDB-21 is relatively smaller dataset as compared to UCF-101-24, overfitting might happen during training our network (on J-HMDB-21) due to the fact that we do not use any expensive data augmentation such as multi-scale technique used in~\cite{peng2016eccv}, resulting relatively lower detection performance.
It is interesting to see how our AMTnet-Flow behaves with multi-scale and multi-region based training.
We keep this extension as a future work.

\subsection{AMTnet-Flow online model evaluation} \label{sec:exp:online}
\SAHA{Gurkirt got some promising results for this section on J-HMDB-21, and the model on UCF-101-24 has been already trained, the evaluation is yet to be done.}\\
\SAHA{The main takeaways in this section are:}\\
\SAHA{1. Online pipeline outperforms the SOA models.}\\ 
\SAHA{2. Our train time conv feature fusion scheme shows better results than the test time late fusion.}\\
\SAHA{3. It is faster than the offline model, and thus, suitable for online real-time applications.}\\

\SAHA{Somewhere you need to explain the AMTnet SSD based motion model, mainly what are the inputs: are they 2 sets of 5  stacked optical flow?}\\

\subsubsection{Ablation study}
In this section, we provide an ablation study of our new AMTnet online action detection framework.
Firstly, we implement AMTnet using SSD network architecture and train the appearance and motion models separately.
Then we apply a late fusion~\cite{} to fuse the appearance and motion cues during test time.
% to extract the detection micro-tubes which can leverage the complementary aspects of both RGB and flow detections.
The output of the late fusion is a set of detection micro-tubes which are then used to incrementally build action tubes in an online fashion using the algorithm of~\cite{}.
In Table~\ref{}, we report the action detection performance (video mAP) of AMTnet appearance, motion and fused models.

\subsubsection{Train time feature fusion}
To show the efficacy of our train time conv feature fusion scheme, 





%---------------------------------------------------------------------------------------
% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
\iffalse
\begin{table}[!t]
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{An Example of a Table}
\label{table_example}
\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{table}
\fi
